ZoDi: Zero-Shot Domain Adaptation with Diffusion-Based Image Transfer

Deep learning models achieve high accuracy in segmentation tasks among others, yet domain shift often degrades the models' performance, which can be critical in real-world scenarios where no target images are available. This paper proposes a zero-shot domain adaptation method based on diffusion models, called ZoDi, which is two-fold by the design: zero-shot image transfer and model adaptation. First, we utilize an off-the-shelf diffusion model to synthesize target-like images by transferring the domain of source images to the target domain. In this we specifically try to maintain the layout and content by utilising layout-to-image diffusion models with stochastic inversion. Secondly, we train the model using both source images and synthesized images with the original segmentation maps while maximizing the feature similarity of images from the two domains to learn domain-robust representations. Through experiments we show benefits of ZoDi in the task of image segmentation over state-of-the-art methods. It is also more applicable than existing CLIP-based methods because it assumes no specific backbone or models, and it enables to estimate the model's performance without target images by inspecting generated images. Our implementation will be publicly available.

==> intro.tex <==
\section{Introduction}
Deep neural networks have greatly advanced the performance of computer vision in various tasks~\cite{NIPS2015-RPN,ronneberger2015unet}. The deep learning-based models typically perform very well when the data distributions are consistent between the domains of training and testing. A well-known downside however is that they may significantly drop when tested on out-of-distribution data~\cite{ovadia2019distributionshift}, which can be critical in real-world application scenarios.

Faced with the issues due to domain-shift, some domain adaptation techniques~\cite{} use images from the target domain in an unsupervised way where the model could access them without labels. There are many attempts for the challenge, such as feature-level adaptation~\cite{long2015featurelevel}, image-level adaptation~\cite{murez2017imagelevel}, and output-level adaptation~\cite{}. Moreover, a few recent research~\cite{benigmim2023datum} addressed even stricter settings, i.e. one-shot unsupervised training where only one target image is accessible by the model. Yet, it is not always possible to obtain one.

\textbf{Zero-shot} domain adaptation in this respect is a promising research direction for reducing the requirement where real images from the target domain are unavailable. Some research~\cite{lengyel2021ciconv,luo2023similarity} introduced zero-shot day-night adaptation. Despite their effectiveness, they are limited to the specific setting.  Other recent work~\cite{vidit2023clipthegap,fahes2023poda} proposed utilizing the text features of prompts from CLIP~\cite{Radford2021-bi}, a vision-language pre-trained model, for addressing more general zero-shot settings. Despite their great results, they require freezing the image backbone of CLIP, which restricts the selection of the backbone and its performance.

% A POSITION SENTENNCE                                                                                      
In this paper, we are also concerned ourselves (?) with zero-shot domain adaptation applicable to general setting but without the restriction. % by using diffusion-based image transfer.                           
In particular, we are interested in the task of segmentation. 
% This research proposes zerO-shOt domain adaptation with Paired Synthetic data (OOPS).     
As illustrated in Fig.~\ref{fig:abstract}, our approach comprises zero-shot image transfer and model adaptation.
Our basic strategy to meet [FIXME: this goal] is to leverage powerful diffusion models~\cite{rombach2022stablediffusion} for zero-shot image transfer of source images to the target domain. 
That is, we first transfer images to the target domain using diffusion models, which involves the challenge of keeping the layout and content. We then train the segmentation models to learn domain-robust representations by maximizing the feature similarity of images from the two domains for better adaptation.

Yet, in this framework, it is non-trivial to change the domain of the images while maintaining the layout and content. For example, some objects in the original images are often eliminated in existing diffusion-based style transfer methods~\cite{hertz2022prompttoprompt,mokady2022nulltext}. As a solution, we propose a novel method where we adopt layout-to-image diffusion models~\cite{zhang2023adding,xue2023freestyle,li2023gligen} and stochastic inversion~\cite{zhang2023inversionbased} for keeping both of the layout and content. 
As for layout-to-image models, we adopt pre-trained ControlNet due to its simplicity. To maintain the information of original images, we use real images as guidance and adapt stochastic inversion techniques proposed in InST. 
Through experiments we show that this image transfer method is capable of changing the image domain with little/no artifacts and improve the performance of the segmentation models.

Since our method does not assume any specific backbone (e.g. CLIP) it is available for existing daytime models, which can be seen as a significant advantage over CLIP-based methods [FIXME: reference]. In order to verify its effectiveness, we conduct various experiments on semantic segmentation in different settings: {\it day to night, clear to adverse weather}, and {\it real to synthetic}. Results [FIXME: add more concrete results] on those settings showcase the gain over existing methods. The contributions of the paper can be summarized as below:

\begin{itemize}
\item We propose a diffusion-based zero-shot domain adaptation method for the first time. It consists of diffusion-based image transfer and similarity-based model adaptation.                                                                                         
\item
We suggest that utilizing layout-to-image diffusion models with stochastic inversion can achieve high-quality image transfer while maintaining the layout and content of the images.
\item Through experiments, we show that using generated images by the layout-to-image models for training segmentation models helps achieve a state-of-the-art performance.

\item Unlike CLIP-based methods, our method does not assume any specific model backbone, which enables acting as a plug-and-play method to other existing daytime models. 
% This is a significant advantage against previous work.       
\end{itemize}
